Performance Comparison of Dual Connectivity and Hard Handover for LTE-5G Tight Integration in mmWave Cellular Networks

MmWave communications are expected to play a major role in the Fifth generation of mobile networks. They offer a potential multi-gigabit throughput and an ultra-low radio latency, but at the same time suffer from high isotropic pathloss, and a coverage area much smaller than the one of LTE macrocells. In order to address these issues, highly directional beamforming and a very high-density deployment of mmWave base stations were proposed. This Thesis aims to improve the reliability and performance of the 5G network by studying its tight and seamless integration with the current LTE cellular network. In particular, the LTE base stations can provide a coverage layer for 5G mobile terminals, because they operate on microWave frequencies, which are less sensitive to blockage and have a lower pathloss. This document is a copy of the Master's Thesis carried out by Mr. Michele Polese under the supervision of Dr. Marco Mezzavilla and Prof. Michele Zorzi. It will propose an LTE-5G tight integration architecture, based on mobile terminals' dual connectivity to LTE and 5G radio access networks, and will evaluate which are the new network procedures that will be needed to support it. Moreover, this new architecture will be implemented in the ns-3 simulator, and a thorough simulation campaign will be conducted in order to evaluate its performance, with respect to the baseline of handover between LTE and 5G.

==> figures/rrc_4_2040.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.04877,0.57722,0.82283}%
\definecolor{mycolor2}{rgb}{0.48712,0.74906,0.48398}%
\definecolor{mycolor3}{rgb}{0.97886,0.82714,0.16331}%
%
\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.5ex}}
\begin{axis}[%
width=0.951\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
xmin=0,
xmax=10,
xlabel={X2/buffer configurations},
xtick={1,2,3,4,5,6,7,8,9,10},
xticklabels={$0.1$ $1$, $1$ $1$, $10$ $1$, $0.1$ $10$, $1$ $10$, $10$ $10$, $0.1$ $100$, $1$ $100$, $10$ $100$, ms MB},
xticklabel style={text width=6, align=center}, xmajorgrids,
ymin=4000,
ymax=11000,
ylabel={RRC traffic (DL) [bit/s]},
ymajorgrids, ylabel shift = -5 pt, yticklabel shift = -3 pt,
axis background/.style={fill=white},
title style={font=\bfseries},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=mycolor1,solid,line width=1.2pt,mark size=1.0pt,mark=o,mark options={solid}]
  table[row sep=crcr]{%
1	5956.11536355189\\
2	5907.08821038964\\
3	4634.39904854762\\
4	5951.31474625188\\
5	5915.62368560416\\
6	4664.27706096\\
7	5951.31474625188\\
8	5915.62368560416\\
9	4662.93763934661\\
};
\addlegendentry{DC, $\lambda=20\mu$s};

\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=star,mark options={solid}]
  table[row sep=crcr]{%
1	10946.8176710963\\
2	10633.5234279021\\
3	8546.26755515031\\
4	10946.8176710963\\
5	10633.5234279021\\
6	8456.35141259265\\
7	10946.8176710963\\
8	10633.5234279021\\
9	8456.35141259265\\
};
\addlegendentry{HH, $\lambda=20\mu$s};

\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=asterisk,mark options={solid}]
  table[row sep=crcr]{%
1	5943.79183053298\\
2	5905.7315456803\\
3	4658.75067414594\\
4	5936.49902727374\\
5	5907.18275562065\\
6	4642.44526209248\\
7	5936.49902727374\\
8	5907.18275562065\\
9	4642.44526209248\\
};
\addlegendentry{DC, $\lambda=40\mu$s};

\addplot [color=mycolor3,solid,line width=1.2pt,mark size=1.0pt,mark=star,mark options={solid}]
  table[row sep=crcr]{%
1	10952.9507534999\\
2	10630.6848586106\\
3	8492.82906962582\\
4	10887.8644734732\\
5	10630.6848586106\\
6	8495.22677175181\\
7	10887.8644734732\\
8	10630.6848586106\\
9	8495.22677175181\\
};
\addlegendentry{HH, $\lambda=40\mu$s};

\end{axis}
\end{tikzpicture}%

==> figures/rrc_4_80160.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.97886,0.82714,0.16331}%
\definecolor{mycolor2}{rgb}{0.04981,0.45857,0.86406}%
\definecolor{mycolor3}{rgb}{0.18013,0.71766,0.64243}%
%
\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.5ex}}
\begin{axis}[%
width=0.951\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
xmin=0,
xmax=10,
xlabel={X2/buffer configurations},
xtick={1,2,3,4,5,6,7,8,9,10},
xticklabels={$0.1$ $1$, $1$ $1$, $10$ $1$, $0.1$ $10$, $1$ $10$, $10$ $10$, $0.1$ $100$, $1$ $100$, $10$ $100$, ms MB},
xticklabel style={text width=6, align=center}, xmajorgrids,
ymin=4000,
ymax=11000,
ylabel={RRC traffic (DL) [bit/s]},
ymajorgrids, ylabel shift = -5 pt, yticklabel shift = -3 pt,
axis background/.style={fill=white},
title style={font=\bfseries},
legend style={legend cell align=left,align=left,draw=white!15!black}
]
\addplot [color=mycolor1,solid,line width=1.2pt,mark size=1.0pt,mark=*,mark options={solid}]
  table[row sep=crcr]{%
1	5949.28843117803\\
2	5907.32793087574\\
3	4645.4579781917\\
4	5954.44870756334\\
5	5907.32793087574\\
6	4642.78093343619\\
7	5954.44870756334\\
8	5907.32793087574\\
9	4642.78093343619\\
};
\addlegendentry{DC, $\lambda=80\mu$s};

\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=+,mark options={solid}]
  table[row sep=crcr]{%
1	10952.9507534999\\
2	10621.4269009507\\
3	8499.60431568643\\
4	10952.9507534999\\
5	10627.6201948363\\
6	8495.07202947351\\
7	10952.9507534999\\
8	10627.6201948363\\
9	8495.07202947351\\
};
\addlegendentry{HH, $\lambda=80\mu$s};

\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=x,mark options={solid}]
  table[row sep=crcr]{%
1	5940.17774926911\\
2	5891.6139190607\\
3	4643.92319069902\\
4	5940.17774926911\\
5	5891.6139190607\\
6	4643.92319069902\\
7	5940.17774926911\\
8	5891.6139190607\\
9	4643.92319069902\\
};
\addlegendentry{DC, $\lambda=160\mu$s};

\addplot [color=mycolor3,solid,line width=1.2pt,mark size=1.0pt,mark=o,mark options={solid}]
  table[row sep=crcr]{%
1	10934.8269356475\\
2	10657.4446920213\\
3	8525.67754097798\\
4	10935.0129821591\\
5	10644.7683010206\\
6	8525.67754097798\\
7	10935.0129821591\\
8	10644.7683010206\\
9	8525.67754097798\\
};
\addlegendentry{HH, $\lambda=160\mu$s};

\end{axis}
\end{tikzpicture}%

==> figures/th_4_2040.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.04877,0.57722,0.82283}%
\definecolor{mycolor2}{rgb}{0.48712,0.74906,0.48398}%
\definecolor{mycolor3}{rgb}{0.97886,0.82714,0.16331}%
%
\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.5ex}}\pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.5ex}}

\begin{axis}[%
width=0.951\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
xmin=0,
xmax=10,
xlabel={X2/buffer configurations},
xmajorgrids,
ymin=180000000,
ymax=300000000,
xtick={1,2,3,4,5,6,7,8,9,10},
xticklabels={$0.1$ $1$, $1$ $1$, $10$ $1$, $0.1$ $10$, $1$ $10$, $10$ $10$, $0.1$ $100$, $1$ $100$, $10$ $100$, ms MB},
xticklabel style={text width=6, align=center},
ylabel={PDCP Throughput [bit/s]},
ymajorgrids, ylabel shift = -5 pt, yticklabel shift = -3 pt,
axis background/.style={fill=white},
title style={font=\bfseries},
legend style={legend cell align=left,align=left,draw=white!15!black}
]

\addplot [color=mycolor1,solid,line width=1.2pt,mark size=1.0pt,mark=o,mark options={solid}]
  table[row sep=crcr]{%
1	277610598.817538\\
2	277102926.755556\\
3	268509426.231578\\
};
\addplot [color=mycolor1,solid,line width=1.2pt,mark size=1.0pt,mark=o,mark options={solid}]
  table[row sep=crcr]{%
4	287859844.348488\\
5	287576476.492929\\
6	279214232.306174\\
};
\addplot [color=mycolor1,solid,line width=1.2pt,mark size=1.0pt,mark=o,mark options={solid}]
  table[row sep=crcr]{%
7	288314559.112124\\
8	288032008.888889\\
9	279836421.037936\\
};
\addlegendentry{DC, $\lambda=20\mu$s};

\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=star,mark options={solid}]
  table[row sep=crcr]{%
1	259763514.562178\\
2	258837002.807789\\
3	260219755.905724\\
};
\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=star,mark options={solid}]
  table[row sep=crcr]{%
4	264029771.750987\\
5	263568190.978342\\
6	264085360.395062\\
};
\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=star,mark options={solid}]
  table[row sep=crcr]{%
7	264484645.789183\\
8	264025932.380525\\
9	264591242.540965\\
};
\addlegendentry{HH, $\lambda=20\mu$s};

\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=asterisk,mark options={solid}]
  table[row sep=crcr]{%
1	197499401.303391\\
2	197083114.392818\\
3	189364967.260001\\
};
\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=asterisk,mark options={solid}]
  table[row sep=crcr]{%
4	201802453.854839\\
5	201608655.237234\\
6	195686725.338873\\
};
\addplot [color=mycolor2,solid,line width=1.2pt,mark size=1.0pt,mark=asterisk,mark options={solid}]
  table[row sep=crcr]{%
7	201802453.854839\\
8	201608655.237234\\
9	195686708.30453\\
};
\addlegendentry{DC, $\lambda=40\mu$s};

\addplot [color=mycolor3,solid,line width=1.2pt,mark size=1.0pt,mark=star,mark options={solid}]
  table[row sep=crcr]{%
1	183529287.351768\\
2	182687179.648618\\
3	183146057.867186\\
};
\addplot [color=mycolor3,solid,line width=1.2pt,mark size=1.0pt,mark=star,mark options={solid}]
  table[row sep=crcr]{%
4	186720903.436251\\
5	186090476.66084\\
6	184928122.458151\\
};
\addplot [color=mycolor3,solid,line width=1.2pt,mark size=1.0pt,mark=star,mark options={solid}]
  table[row sep=crcr]{%
7	186720903.436251\\
8	186090476.66084\\
9	184928122.458151\\
};
\addlegendentry{HH, $\lambda=40\mu$s};
       
\end{axis}
\end{tikzpicture}%

==> frontmatter/abbr.tex <==
\begin{abbreviations}

\item[ABF] Analog Beamforming
\item[AM] Acknowledged Mode
\item[AMC] Adaptive Modulation and Coding
\item[AoA] Angle of Arrival
\item[AoD] Angle of Departure
\item[BLER] Block Error Rate
\item[BS] Base Stations
\item[CB] Code Block
\item[CDF] Cumulative Distribution Function
\item[C-RNTI] Cell Radio Network Temporary Identifier
\item[CQI] Channel Quality Indicator
\item[CRT] Complete Report Table
\item[CSI] Channel Side Information
\item[DBF] Digital Beamforming
\item[DC] Dual Connectivity
\item[DL] Downlink
\item[DRB] Data Radio Bearer
\item[eNB] evolved Node Base
\item[EPC] Evolved Packet Core
\item[EPS] Evolved Packet System
\item[E-RAB] E-UTRAN Radio Access Bearer
\item[E-UTRAN] Evolved Universal Terrestrial Radio Access Network
\item[FDD] Frequency Division Duplexing
\item[FS] Fast Switching
\item[GTP] GPRS Tunneling Protocol
\item[HARQ] Hybrid Automatic Repeat reQuest
\item[HBF] Hybrid Beamforming
\item[HH] Hard Handover
\item[IA] Initial Access
\item[IMSI] International Mobile Subscriber Identity
\item[ITU] International Telecommunication Union
\item[LOS] Line of Sight
\item[MAC] Medium Access Control
\item[MCG] Master Cell Group
\item[MCS] Modulation and Coding Scheme
\item[MeNB] Master eNB
\item[METIS] Mobile and wireless communications Enablers for the Twenty-twenty Information Society
\item[MIB] Master Information Block
\item[MICB] Mutual Information per Coded Bit
\item[MIMO] Multiple Input Multiple Output
\item[MME] Mobility Management Entity
\item[MMIB] Mean Mutual Information per coded Bit
\item[MTU] Maximum Transfer Unit
\item[NLOS] Non Line of Sight
\item[NYU] New York University
\item[OFDM] Orthogonal Frequency Division Multiplexing 
\item[OFDMA] Orthogonal Frequency-Division Multiple Access
\item[PDCP] Packet Data Convergence Protocol
\item[PDU] Packet Data Unit
\item[P-GW] Packet Gateway
\item[PHY] Physical
\item[QoE] Quality of Experience
\item[RA] Random Access
\item[RAN] Radio Access Network
\item[RAT] Radio Access Technology
\item[RLC] Radio Link Control
\item[RLF] Radio Link Failure
\item[RMS] Root Mean-Squared
\item[RRC] Radio Resource Control
\item[RT] Report Table
\item[SCG] Secondary Cell Group
\item[SDN] Software Defined Networking
\item[SDU] Service Data Unit
\item[SeNB] Secondary eNB
\item[S-GW] Service Gateway
\item[SI] System Information
\item[SIB] System Information Block
\item[SRB] Signalling Radio Bearer
\item[TB] Transport Block
\item[TDD] Time Division Duplexing 
\item[TDMA] Time Division Multiple Access
\item[TM] Transparent Mode
\item[UE] User Equipment
\item[UL] Uplink
\item[ULA] Uniform Linear Array
\item[UM] Unacknowledged Mode

\end{abbreviations}

==> frontmatter/abstract.tex <==
%!TEX root = ../dissertation.tex
% the abstract

MmWave communications are expected to play a major role in the Fifth generation of mobile networks. They offer a potential multi-gigabit throughput and an ultra-low radio latency, but at the same time suffer from high isotropic pathloss, and a coverage area much smaller than the one of LTE macrocells. In order to address these issues, highly directional beamforming and a very high-density deployment of mmWave base stations were proposed. This Thesis aims to improve the reliability and performance of the 5G network by studying its tight and seamless integration with the current LTE cellular network. In particular, the LTE base stations can provide a coverage layer for 5G mobile terminals, because they operate on microWave frequencies, which are less sensitive to blockage and have a lower pathloss. 

This Thesis will propose an LTE-5G tight integration architecture, based on mobile terminals' dual connectivity to LTE and 5G radio access networks, and will evaluate which are the new network procedures that will be needed to support it. Moreover, this new architecture will be implemented in the ns--3 simulator, and a thorough simulation campaign will be conducted in order to evaluate its performance, with respect to the baseline of handover between LTE and 5G.

==> frontmatter/abstract_compact.tex <==
%!TEX root = ../dissertation.tex
% the abstract

\textbf{Abstract } -- MmWave communications are expected to play a major role in the Fifth generation of mobile networks. They offer a potential multi-gigabit throughput and an ultra-low radio latency, but at the same time suffer from high isotropic pathloss, and a coverage area much smaller than the one of LTE macrocells. In order to address these issues, highly directional beamforming and a very high-density deployment of mmWave base stations were proposed. This Thesis aims to improve the reliability and performance of the 5G network by studying its tight and seamless integration with the current LTE cellular network. In particular, the LTE base stations can provide a coverage layer for 5G mobile terminals, because they operate on microWave frequencies, which are less sensitive to blockage and have a lower pathloss. 

This document is a copy of the Master's Thesis carried out by Mr. Michele Polese under the supervision of Dr. Marco Mezzavilla and Prof. Michele Zorzi. It will propose an LTE-5G tight integration architecture, based on mobile terminals' dual connectivity to LTE and 5G radio access networks, and will evaluate which are the new network procedures that will be needed to support it. Moreover, this new architecture will be implemented in the ns--3 simulator, and a thorough simulation campaign will be conducted in order to evaluate its performance, with respect to the baseline of handover between LTE and 5G.

==> frontmatter/authorlist.tex <==
%!TEX root = ../dissertation.tex
\noindent The following authors contributed to Chapter 1: Albert Einstein, George Gamow and Pief Panofsky.

\noindent The following authors contributed to Chapter 2: I. I. Rabi, Niels Bohr and Norman Ramsey.

\noindent The following authors contributed to Chapter 3: Ramon y Cajal, Andrew Huxley.


==> frontmatter/dedication.tex <==
%!TEX root = ../dissertation.tex
% dedication text

A chi mi sostiene da sempre.

==> frontmatter/preface.tex <==
%!TEX root = ../dissertation.tex
% the acknowledgments section

La quinta generazione di reti cellulari prevede l'utilizzo di comunicazioni su frequenze millimetriche. Queste, infatti, offrono una potenziale capacità nell'ordine del gigabit, e una latenza estremamente ridotta. Tuttavia, la perdita di potenza del segnale trasmesso dovuta alla propagazione è molto alta, e la copertura di una cella con frequenze così elevate è ridotta. Per ovviare a questi problemi, si propone di utilizzare tecniche di beamforming e un'installazione ad alta densità di stazioni radio base per il 5G. Questa tesi propone un'ulteriore soluzione per migliorare l'affidabilità e le prestazioni della rete 5G, studiando una possibile integrazione con l'attuale rete LTE. In particolar modo, le stazioni radio LTE possono offrire una copertura omogenea alle celle 5G, in quanto usano frequenze più basse e meno soggette a diminuzione della potenza del segnale per la propagazione.

Questa tesi propone una architettura per l'integrazione di LTE e 5G, basata su terminali connessi contemporaneamente alla rete LTE e 5G, e valuta quali sono le procedure di rete necessarie per supportarla. Inoltre, questa architettura sarà implementata nel simulatore di rete ns--3 e una estensiva campagna di simulazioni fornirà risultati utili alla valutazione delle prestazioni del sistema, rispetto a quelle del caso di riferimento con handover tra le due reti. 


==> frontmatter/thanks.tex <==
%!TEX root = ../dissertation.tex
% the acknowledgments section

Vorrei ringraziare i miei genitori, che mi supportano da sempre, in tutte le scelte che faccio. Ringrazio Marta, per il sostegno, la pazienza e la condivisione di gioie e preoccupazioni.

Desidero ringraziare il Prof. Michele Zorzi, e Marco Mezzavilla, per avermi dato l'opportunità di lavorare nell'ambito del 5G e per avermi messo in contatto con i settori più avanzati della ricerca nelle telecomunicazioni. Grazie anche al Prof. Andrea Zanella, per la fiducia nello scegliermi come tutor, e a Marco Centenaro, per tutti i consigli.

Grazie a tutti i coinquilini e condomini di Via Manara, e a Davide, per il tempo passato insieme in questi anni patavini, e non solo. Grazie ai compagni di mensa, homework e studio in Da: Davide, Paolo, Andrea, Silvia, Alberto, Alberto, Gianluca, Marco, Laura, Beatrice, Marchino, Riccardo e Nicola. Grazie ai GpO e agli amici musicisti, Erin in particolare, per i fantastici momenti passati insieme.

I would like to thank also Prof. Sundeep Rangan, Russell Ford and Menglei Zhang from NYU, and M\aa rten Ericson from Ericsson, for their precious help and advice.

